Strategic Facility Location via Predictions

The facility location with strategic agents is a canonical problem in the literature on mechanism design without money. Recently, Agrawal et. al. considered this problem in the context of machine learning augmented algorithms, where the mechanism designer is also given a prediction of the optimal facility location. An ideal mechanism in this framework produces an outcome that is close to the social optimum when the prediction is accurate (consistency) and gracefully degrades as the prediction deviates from the truth, while retaining some of the worst-case approximation guarantees (robustness). The previous work only addressed this problem in the two-dimensional Euclidean space providing optimal trade-offs between robustness and consistency guarantees for deterministic mechanisms. We consider the problem for \emph{general} metric spaces. Our only assumption is that the metric is continuous, meaning that any pair of points must be connected by a continuous shortest path. We introduce a novel mechanism that in addition to agents' reported locations takes a predicted optimal facility location $\hat{o}$. We call this mechanism $\texttt{Harmonic}$, as it selects one of the reported locations $\tilde{\ell}_i$ with probability inversely proportional to $d(\hat{o},\tilde{\ell}_i)+ \Delta$ for a constant parameter $\Delta$. While \harm \ mechanism is not truthful, we can \emph{characterize the set of undominated strategies} for each agent $i$ as solely consisting of the points on a shortest path from their true location $\ell_i$ to the predicted location $\hat{o}$. We further derive \emph{consistency and robustness guarantees on the Price of Anarchy (PoA)} for the game induced by the mechanism.

==> mechanism.tex <==
\section{Problem Definition and Notation}






TBD: remark on our model why not mixed. computational issue. expectation of ratios. extending meric to continuous domain..


\paragraph{Our Results.} As mentioned before, we ideally would like to design a strategy-proof mechanism. It is known that choosing a facility from the reported locations uniformly at random is strategy-proof and is a 2-approximation. In fact, 2-approximation is the best one can hope for even in a tree metric \cite{alon2010strategyproof}. 
(TBD: Sungjin. I doin't think this statement is true. It is conjectured to be the barrier. And, there is no $1+\eps$-startegy-proof approxiamtion known)
Here, we would like to break this 2-approximation barrier with the aid of the predictions $\po$ and $\pa$. We would like to have a nearly optimum solution when $\po$ and $\pa$ are close to their real location/quantity. 


One could try to achieve this is by outputting $\po$ with probability $1 - \eps$ and run the 2-approximate uniform sampling otherwise, but it has the following issue. The resulting expected cost will be 
$$(1 - \eps) \cdot d(\po, o) + 2\eps \ \opt, $$
where $\opt$ denotes the optimum cost.
Most importantly, the mechanism is not robust because, for any fixed $\eps$, the cost can be much larger than $\opt$ when $d(\po, o) \gg \opt$. Further, the uniform sampling can be severely affected by a single agent. To see this, consider an instance where $n-1$ points are at the same location and the other is at a distance $D$ from them. Then, assuming $n$ is sufficiently large, it's easy to see that $\opt \approx \frac{D}{n}$ while the uniform sampling has a standard deviation of $\frac{D}{\sqrt n}$. \snote{Is it known that Harmonic is less susceptible to few agents? Then, we should cite it.}


\snote{It will be nice to have a lower bound showing that with $\po$ prediction along, we cannot have a strategy-proof mechanism with $1+\eps$-consistency and $O(1_\eps)$-robustness. Should be okay to assume that each agent can report either its true location or $\po$.}

This finding motivates us to use another parameter $\pa$.
(TBD: this logic is not natural.)
We believe that this parameter is easy to predict as it's the \emph{average} distance to agents' true locations, and we will see that we only need to estimate this within $O(1)$ factor. This should be doable by using a third-party information. 

With this extra parameter, we study a variant of harmonic mechanism, which samples $\rl_i$ in inverse proportional to $d(\rl_i, \po) + \pa$. Unfortunately, this mechanism is not truthful, strictly speaking. However, it turns out that if an agent lies, it only benefits all agents. This motivates us to study how far the Nash equilibrium is from the optimum, namely the price of anarchy under this new mechanism. We show that one can achieve $(1+\eps)$-consistency and $O(1 / \eps)$-robustness as long as $\pa$ is a constant approximation of its true value. Although we do not achieve complete robustness in the sense that the solution quality depends on $\pa$, we believe learning $\pa$ is much easier than $\po$ because $\pa$ is the average distance, which is just a single scalar.

\snote{TBD: Tightness of the lower bound.}
\snote{Is it possible to show that complete robustness is impossible to achieve?}




\section{Harmonic Mechanism}





\subsection{Characterizing Dominant Strategies}
We first describe the set of strictly dominant strategies of each agent $i$ under \harm\ mechanism. 
For notational brevity, we will use $\ell_j$ for $j \neq i$ in place of $\rl_j$ because we will study a fixed agent $i$'s strategy for all possible reports of the other agents and we can pretend that $\locsmi$ is a variable vector to agent $i$. \snote{$\leftarrow$ Does this make sense?}







\subsection{Pure vs. Mixed Equilibria}

Note that Claim~\ref{cl:pure_equilibrium} only holds for deterministic locations $\locs$ and no longer holds, if agents use randomized strategies. This is because the denominator $\denomr$ in equation~\eqref{eq:cost_difference} depends on $y=d(\rli,\po)$ and, hence, the expectation in equation~\eqref{eq:cost-of-i} should be taken over $\frac{1}{\denomr(y)}\Big(x+y+\pa-\cost_i(\ell_i,\locsmi)\Big)$. 




We note that while for general $\metric$ the set of pure equlibria of \harm\ mechanism may be empty and a mixed equilibria may be the only available alternative, Claim~\ref{cl:Pure_Nash_existence} is still useful and can be applied even for discrete metric space $\metric$.
\paragraph{Pure vs. Mixed equilibria.} Consider the following observations:
\begin{enumerate}
    \item We could let agents in \harm\ mechanism to explicitly report their locations as randomization between a finite number of points in $\metric$. I.e., we use an extension of the metric space $\metric$ to a larger metric space $\overline{\metric}$ over all finite convex combinations $\overline{\metric}=\{ \boldsymbol{\alpha}=\sum_{i\in[k]}\alpha_i\cdot\ell_i ~|~ \sum_{i\in[k]}\alpha_i=1,~\alpha_i\ge 0,~\ell_i\in\metric\}$;
    a naturally induced metric in $\overline{\metric}$ is given by the Wasserstain distance between two probability distributions $\boldsymbol{\alpha},\boldsymbol{\beta}$ over points in $\metric$.
    \item Pure equilibrium does not exist in general $\metric$, while mixed equilibria always exist.
    \item However, it is often hard to find the best response against randomized strategies of others in the game induced by \harm\ mechanism. Specifically, agent $i$ needs to compute the ratio \eqref{eq:cost-of-i} for all realizations of $\locsmi$. 
    \item Both of the above issues can be alleviated to some degree by extending $\metric$ into a larger metric $\overline{\metric}$ and then considering pure equilibria in $\overline{\metric}$. Indeed, a
    pure equilibrium does exist in $\overline{\metric}$. Also, 
    when many agents participate in \harm\ mechanism, a reasonable 
    approximation/simplification of their expected costs (due to 
    good concentration) can be done by calculating expectations of 
    the numerator and denominator in \eqref{eq:cost-of-i} 
    separately and then using ratio of expectations instead of 
    expected ratio. This approach corresponds exactly to agents 
    playing pure strategies in $\overline{\metric}$.
\end{enumerate}

In conclusion, the outcomes of \harm\ mechanism are perhaps best described by the set of pure Nash equilibria in $\metric$ or $\overline{\metric}$. 





















































    








==> notations.tex <==
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation*}}
\newcommand{\eeq}{\end{equation*}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\minimize}{\mathop{\rm minimize}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bs}{\mathbf s}
\newcommand{\SW}{\textsc{SW}}
\newcommand{\Rev}{\textsc{Rev}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\tempp}{\tilde{p}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ind}[1]{\mathbb{I}\left[\vphantom{\sum}#1\right]}

\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand*{\hm}[1]{#1\nobreak\discretionary{}%
{\hbox{$\mathsurround=0pt #1$}}{}}

\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}%
\newcommand{\Ex}[2][]{\operatorname{\mathbb E}_{#1}\InBrackets{#2}}
\newcommand{\Exlong}[2][]{\operatornamewithlimits{\mathbb E}\limits_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\newcommand{\Prlong}[2][]{\operatornamewithlimits{\mathbf{Pr}}\limits_{#1}\InBrackets{#2}}
\newcommand{\Var}[2][]{\operatorname{\mathbf{Var}}_{#1}\InBrackets{#2}}
\newcommand{\Varlong}[2][]{\operatornamewithlimits{\mathbf{Var}}\limits_{#1}\InBrackets{#2}}
\newcommand{\eqdef}{\overset{\mathrm{def}}{=\mathrel{\mkern-3mu}=}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\iprod}[2]{\langle #1, #2 \rangle}
\newcommand\restr[2]{{%
  \left.\kern-\nulldelimiterspace %
  #1 %
  \vphantom{\big|} %
  \right|_{#2} %
  }}
\def\prob{\Prx}
\def\Prl{\Prlong}
\def\expect{\Ex}

\newcommand{\setmi}[1][i]{\ensuremath{S_{\text{-}#1}}}
\newcommand{\oset}{\ensuremath{\widetilde{S}}}




\newcommand{\metric}{\mathcal{M}}
\newcommand{\elli}[1][i]{\ell_{#1}}
\newcommand{\ells}{\ensuremath{\boldsymbol\ell}}
\newcommand{\ellsmi}[1][i]{\ells_{\text{-}#1}}
\DeclareMathOperator{\SC}{\textsf{SC}}
\DeclareMathOperator{\cost}{\textsf{cost}}
\newcommand{\costi}[1][i]{\cost_{#1}}
\newcommand{\mcosti}[1][i]{\widetilde{\cost}_{#1}}

\newcommand{\fclts}{\vect{f}}
\newcommand{\installeds}[1][s]{\fclts_{[#1]}}
\newcommand{\alg}{\textsf{alg}}
\newcommand{\algname}{\texttt{Proportional}}
\newcommand{\algnameshort}{\texttt{On-Prop}}
\newcommand{\aval}[1]{\alg\InParentheses{#1}}
\newcommand{\abound}[1]{\Phi\InParentheses{#1}}

\newcommand{\vs}{\vect{s}}
\newcommand{\vu}{\vect{u}}
\newcommand{\vusmi}[1][i]{\vect{u}_{\text{-}#1}}

\newcommand{\hui}[1][i]{\hat{u}_{#1}}
\newcommand{\hsi}[1][i]{\hat{s}_{#1}}
\newcommand{\hvs}{\vect{\hat{s}}}
\newcommand{\hvusmi}[1][i]{\vect{\hat{u}}_{\text{-}#1}}
\newcommand{\hvu}{\vect{\hat{u}}}


\newcommand{\opt}{\textsf{opt}}
\newcommand{\optk}[1][k]{\textsf{opt}_{#1}}
\newcommand{\os}{\vect{o}}
\newcommand{\distset}{\mathcal{F}}
\newcommand{\dist}{\mathcal{D}}



